Unsupervised Boosting-based Autoencoder Ensembles for Outlier Detection

Autoencoders, as a dimensionality reduction technique, have been recently applied to outlier detection. However, neural networks are known to be vulnerable to overfitting, and therefore have limited potential in the unsupervised outlier detection setting. Current approaches to ensemble-based autoencoders do not generate a sufficient level of diversity to avoid the overfitting issue. To overcome the aforementioned limitations we develop a Boosting-based Autoencoder Ensemble approach (in short, BAE). BAE is an unsupervised ensemble method that, similarly to the boosting approach, builds an adaptive cascade of autoencoders to achieve improved and robust results. BAE trains the autoencoder components sequentially by performing a weighted sampling of the data, aimed at reducing the amount of outliers used during training, and at injecting diversity in the ensemble. We perform extensive experiments and show that the proposed methodology outperforms state-of-the-art approaches under a variety of conditions.

==> appunti.tex <==


%%%%%%% .  POSSIBLE FUTURE WORKS:
Without loss of generalization, one can adaptively vary the base architecture at each iteration. Nevertheless, in this paper we maintain a static architecture to interpret the impact of other hyper-parameters.


%%%%  FLOW BY DOMENICONI
{\color{red} Outline [Carlotta]

Overall idea and motivation:\\

- building a cascade of autoencoders a-la-boosting, where the sample provided in input to the (j+1)-th component depends on the j-th component

- How do we define a distribution over the data to guide the sampling? describe how an autoencoder operates; the nature of outliers and why we expect outliers to receive higher reconstruction error; from this follows the idea of defining a distribution that assigns weights to data which are inversely proportional to the corresponding reconstruction error.

- Argue how this generates diverse components.

- Then provide necessary notation and definitions and give a pseudo-code of the algorithm.

All the details about the specific architecture we use go in the Experimental Section.

{\bf Eliminate the references to bagging. We are not using bagging!!}
}



%%%%%%%%%%%%%%%%% SHORT BULLET %%%%%%%%%%%%%%%

\begin{itemize}
    \item Standard UCI ML datasets + big (ALOI, KDD, MNIST)
    
     \item sensitivity test on the number of components shows that our strategy with 20 components shows the optimum depth of the boosting cascade.
    \item Comparison with SOTA: RandNet (deep outlier detection ensemble with random connections) and the method in Hawkins
    
    \item comparison with classic anomaly detection algos such as HiCS, LOF, 1-class SVM, isolation forest
   
    \item under different consensus functions we still have greater AUCPR than the other approaches
    
    \item the AUCPR for the different runs of our method are statistically more significant than the others in the majority of the datasets
    
    \item We perform way better in the bigger datasets
\end{itemize}
\end{abstract}



%%%%%%%%%% Outlier vs Inlier Discussion %%%%%%%%

{\color{red}{[I am leaning to delete the following text in green]}}
{\color{green}
Another possibility is to design a probability function that gives sampling priority to the outliers. Nevertheless, this solution might lead to an oscillating behavior where the learning of each iteration is focused first on inliers and then on the outliers. To better understand this oscillating behavior consider the following scenario. Suppose we have three data-points $\mathbf{X}^0=\{a,b,c\}$ where $a$ is an outlier and $b$ and $c$ are inliers. The training of the first \aaa \xspace produces a reconstruction error of $a$ that is higher than the error of $b$ and $c$ (the learning is focused now on the inliers). The next iteration is based on the dataset $\mathbf{X}^1=\{a,a,b\}$ and thus it learns a better representation of $a$ (outliers). Consequently, the reconstruction errors of $b$ and $c$ are higher than the error of $a$ and in the subsequent iteration the dataset consists of $\mathbf{X}^2=\{b,c,c\}$ focusing the learning process again on the inliers.
\todo[inline]{It is possible to add a visual example to clarify much more.}}

==> sec_intro.tex <==
% !TEX root = main.tex
\section{Introduction}

\todo[inline]{B: my modifications don't suggest a definitive draft. I'm just suggesting a way of writing which might be wrong. Feel free to change anything. Grammarly suggests to use an active form of verbs for better engagement.}
\todo[inline]{G: Motiation Boosting,
Releated Work Bias and Variance: Randnet agisce solo su variance mentre noi anche su bias. Definire il rec_err 

Challenge: non è semplice portare boosting in un contesto unsupervised. + AE

Motivazione metodi classici vs nostro quando le dimensionalità sono grandi. Siamo quasi uguali con IF sui dataset classici.


Titolo: Boosting DAE ensemble for Outliers Detection

algoritmo: Boosting AE Ensemble
X : data iniziale |X| = n
S_1 = X primo sample per il primo AE
for j = 2 to m:
    S_j = X samplato all'iterazione j
}




Outlier (anomaly) detection is an unsupervised task which consists of pinpointing irregular patterns in a set of data. Several anomaly detection techniques based on distance \cite{angiulli2002fast,knox1998algorithms,ramaswamy2000efficient}, density \cite{breunig2000lof}, and dimensionality reduction have been proposed. More recently, auto-encoders have shown promising results in identifying anomalies.

\todo{B: I've reformulated a bit the paragraph in order to provide a more natural flow} An auto-encoder (AE) is a symmetric multi-layered neural network that learns to reconstruct the input. In other words, an AE generates a compressed input representation. Meanwhile the reduced data image represents the majority of instances (i.e. inliers), it models outliers (i.e. examples of unusual patterns) less accurately. Hence, outliers have more eminent reconstruction errors that serve as measurements for outlierness scores. Because outliers disturb the distribution of data, an AE experiences flaws during the learning phase, thus generating an erroneous compressed data representation for the inlier examples.

Therefore, we propose a boosting-based AE ensemble strategy to tackle both the anomaly detection task and the correct learning of the pseudo-identity function that maps inlier data. 

\todo[inline]{FINO A QUI CORRETTO!}



%An auto-encoder (AE) is a symmetric multi-layered neural network that tries to reconstruct the input.
%is intended to reconstruct the input layer in the output layer. 
%In other words, an AE provides a reduced dimensionality representation of the data. The basic idea of using an AE for outlier detection is that the model will learn a reduced representation of the majority of the data points and outliers will be less accurately modeled using this representation. Outliers will produce higher reconstruction errors and therefore we can consider reconstruction errors as degree of outlierness.

%Auto-encoders are known to be prone to over-fitting to the outliers which are also included in the training data due to the unsupervised nature of the anomaly detection problem. 
%Ensemble methods are generally employed to evade the dependency of a model on on data locality and data set characteristics. 
%Our basic idea is to move towards reducing the number of outliers present in the training process, by sampling the training data and also 

In this paper, we propose a sampling algorithm to tackle the outlier overfitting problem. At each step, our algorithm sub-samples the original dataset by excluding the outlier instances. In more detail, we initially train a simple AE on the entire dataset which . This model produces outlier scores for the input.

%In this paper we propose a method to directly tackle the overfitting problem by sampling the training data such that we move towards excluding outliers from the training data in an unsupervised setting. 


Our basic idea is that we initially train a simple Auto-encoder on all of the data and generate an outlier score for each datum based on the reconstruction errors obtained from this Auto-encoder. At this point, we sample a new set of training data from the initial set, such that we assign a higher probability of including the data with lower outlier score. The new training set, generally has fewer outliers compared to the initial set, depending on the accuracy of the initial model. The new trained model yields a new set of outlier scores and we can redo the sampling process based on new outlier scores and train another model. We repeat this procedure multiple times and build an ensemble of the constructed models. 
Benefits gained from this ensemble based approach is twofold: first, the weighted sampling generally minimizes the number of outliers in the sample which reduces the negative effect of presence of the outliers in training; second, multiple samplings yields diverse training data for every component, each one contaminated with a different subset of outliers. This injects diversity to the ensemble and helps to avoid overfitting.



==> table_diversity_col.tex <==
% !TEX root = main.tex

\begin{table}[ht]
\centering
\begin{adjustbox}{width=0.6\columnwidth}

\begin{tabular}{lll}
  \hline
Data set & RandNet & \algo \\
\hline
\textbf{ALOI} & 0.223 & \textbf{0.254}\\
\textbf{Ecoli4} & 0.116 & \textbf{0.144}\\
\textbf{Glass} & 0.037 & \textbf{0.095}\\
\textbf{KDD99} & \textbf{0.575} &  0.283 \\
\textbf{Lympho} & 0.275 & \textbf{0.294}\\
\textbf{PageBlocks} & \textbf{0.383} & 0.205\\
\textbf{Pima} & 0.048 & \textbf{0.066}\\
\textbf{SatImage} & \textbf{0.441} & 0.222\\
\textbf{Shuttle} & 0.027 & \textbf{0.085}\\
\textbf{SpamBase} & 0.01 & \textbf{0.042}\\
\textbf{Stamps} & 0.063 & \textbf{0.084}\\
\textbf{WDBC} & \textbf{0.11} & \textbf{0.095}\\
\textbf{Wilt} & \textbf{0.143} & \textbf{0.133}\\
\textbf{WPBC} & 0.033 & \textbf{0.275}\\
\textbf{Yeast05679v4} & \textbf{0.144} & 0.119\\
\textbf{Yeast2v4} & \textbf{0.121} & 0.096\\
\hline
\textbf{MNIST0} & 0.25 & \textbf{0.263}\\
\textbf{MNIST1} & \textbf{0.284} & 0.252\\
\textbf{MNIST2} & \textbf{0.287} & 0.245\\
\textbf{MNIST3} & \textbf{0.244} & 0.228\\
\textbf{MNIST4} & \textbf{0.236} & \textbf{0.234}\\
\textbf{MNIST5} & \textbf{0.283} & 0.211\\
\textbf{MNIST6} & \textbf{0.245} & 0.228\\
\textbf{MNIST7} & \textbf{0.214} & 0.197\\
\textbf{MNIST8} & \textbf{0.246} & 0.205\\
\textbf{MNIST9} & \textbf{0.23} & 0.212\\
\end{tabular}
\end{adjustbox}
\caption{ Comparison ensemble diversity generated by RandNet and \algo methods. }
\label{tab:diversity}
\end{table}


==> tables_not_used.tex <==
% \begin{table}[h]
%   \centering
%       \begin{adjustbox}{width=0.9\columnwidth}
%       \setlength\tabcolsep{4.0pt} 
%     \begin{tabular}{l c | c | c | c | c | c | c |}
% Datasets & Lof & RandNet & full-opt & OCSVM & IF & Hawkins\\
% \hline

% \textbf{Ecoli4} & 0.054 & 0.094 & \textbf{0.16} & 0.123 & \textbf{0.175} & 0.121\\
% \textbf{Glass} & \textbf{0.159} & 0.092 & 0.123 & 0.077 & \textbf{0.164} & 0.105\\
% \textbf{Lympho} & 0.486 & 0.856 & \textbf{0.967} & 0.799 & \textbf{0.987} & 0.232\\
% \textbf{PageBlocks} & 0.252 & 0.21 & \textbf{0.314} & 0.238 & 0.244 & \textbf{0.296}\\
% \textbf{Pima} & 0.019 & 0.031 & 0.035 & 0.028 & \textbf{0.043} & 0.03\\
% \textbf{SatImage} & 0.21 & 0.572 & 0.68 & 0.523 & \textbf{0.813} & 0.296\\
% \textbf{Shuttle} & \textbf{0.115} & 0.021 & 0.021 & 0.022 & 0.076 & 0.037\\
% \textbf{SpamBase} & 0.07 & 0.058 & 0.059 & 0.066 & \textbf{0.16} & 0.06\\
% \textbf{Stamps} & 0.099 & 0.128 & \textbf{0.138} & 0.117 & \textbf{0.132} & \textbf{0.142}\\
% \textbf{WDBC} & 0.548 & \textbf{0.592} & \textbf{0.567} & \textbf{0.596} & \textbf{0.658} & 0.49\\
% \textbf{Wilt} & \textbf{0.073} & 0.012 & 0.013 & 0.014 & 0.016 & 0.012\\
% \textbf{WPBC} & 0.211 & 0.221 & \textbf{0.239} & 0.226 & 0.23 & 0.215\\
% \textbf{Yeast05679v4} & 0.136 & 0.109 & \textbf{0.181} & 0.155 & 0.148 & 0.114\\
% \textbf{Yeast2v4} & 0.148 & 0.26 & \textbf{0.371} & \textbf{0.359} & 0.319 & 0.231\\
% \end{tabular}
%   \end{adjustbox}
%   \caption{ \label{tab:baselines}}
% %  \vspace{-2em}
%   \label{ens-size}
% \end{table}


% \vspace{40mm}


% \begin{table}
%   \centering
%       \begin{adjustbox}{width=0.9\columnwidth}
%       \setlength\tabcolsep{4.0pt} 
%     \begin{tabular}{l c | c | c | c | c |  }
% Datasets & LOF & RandNet & Full Opt & OCSVM  \\
% \hline
% \textbf{Ecoli4} & 0.054 & 0.093 & \textbf{0.16} & 0.123\\
% \textbf{Glass} & \textbf{0.159} & 0.092 & 0.123 & 0.077\\
% \textbf{Lympho} & 0.486 & 0.839 & \textbf{0.967} & 0.799\\
% \textbf{PageBlocks} & 0.252 & 0.212 & \textbf{0.314} & 0.238\\
% \textbf{Pima} & 0.019 & 0.031 & \textbf{0.035} & 0.028\\
% \textbf{SatImage} & 0.21 & 0.525 & \textbf{0.68} & 0.523\\
% \textbf{Shuttle} & \textbf{0.115} & 0.021 & 0.021 & 0.022\\
% \textbf{SpamBase} & \textbf{0.07} & 0.058 & 0.059 & \textbf{0.066}\\
% \textbf{Stamps} & 0.099 & 0.128 & \textbf{0.138} & 0.117\\
% \textbf{WDBC} & \textbf{0.548} & \textbf{0.592} & \textbf{0.567} & \textbf{0.596}\\
% \textbf{Wilt} & \textbf{0.073} & 0.012 & 0.013 & 0.014\\
% \textbf{WPBC} & 0.211 & 0.221 & \textbf{0.239} & 0.226\\
% \textbf{Yeast05679v4} & 0.136 & 0.111 & \textbf{0.181} & 0.155\\
% \textbf{Yeast2v4} & 0.148 & 0.261 & \textbf{0.371} & 0.359\\
% \end{tabular}
%   \end{adjustbox}
%   \caption{ \label{tab:baselines}}
%   \vspace{-2em}
%   \label{ens-size}
% \end{table}


% \begin{table}[h]
%   \centering
%       %\begin{adjustbox}{width=0.9\columnwidth}
%       %\setlength\tabcolsep{4.0pt} 
%     \begin{tabular}{l c | c   }

%     Data set & $\frac{1}{x}$ & $\frac{1}{log(x)}$ \\
%     \hline
%     \textbf{Ecoli4} & 0.122 & \textbf{0.126}\\
% \textbf{Glass} & \textbf{0.125} & 0.115\\
% \textbf{Lympho} & \textbf{0.935} & 0.931\\
% \textbf{PageBlocks} & 0.206 & \textbf{0.265}\\
% \textbf{Pima} & \textbf{0.036} & 0.034\\
% \textbf{SatImage} & 0.779 & \textbf{0.803}\\
% \textbf{Shuttle} & \textbf{0.021} & 0.021\\
% \textbf{SpamBase} & 0.059 & \textbf{0.06}\\
% \textbf{Stamps} & \textbf{0.138} & 0.131\\
% \textbf{WDBC} & \textbf{0.586} & 0.584\\
% \textbf{Wilt} & \textbf{0.013} & 0.013\\
% \textbf{WPBC} & \textbf{0.237} & 0.232\\
% \textbf{Yeast05679v4} & \textbf{0.163} & 0.162\\
% \textbf{Yeast2v4} & \textbf{0.371} & 0.368\\
%   \end{tabular}
% %  \end{adjustbox}
%   \caption{ Comparison of $\frac{1}{x}$ and $\frac{1}{log(x)}$ as weighting functions
%   \label{tab:old_new}}
%   \vspace{-2em}
%   \label{ens-size}
% \end{table}


% %%%%%%
% \begin{figure}[!htbp]
% \begin{subfigure}[b]{\columnwidth}
% 	\includegraphics[width=0.9\columnwidth,height=]{SatImage.jpeg}
% 	\label{fig:comp_dist:b}
% \end{subfigure}  
% \begin{subfigure}[b]{\columnwidth}
% 	\includegraphics[width=0.9\columnwidth]{SpamBase.pdf}
% 	\label{fig:comp_dist:c}
% \end{subfigure}  
% \begin{subfigure}[b]{\columnwidth}
% 	\includegraphics[width=0.9\columnwidth]{Wilt.pdf}
% 	\label{fig:comp_dist:d}
% \end{subfigure}  
% \begin{subfigure}[b]{\columnwidth}
% 	\includegraphics[width=0.9\columnwidth]{WPBC.pdf}
% 	\label{fig:comp_dist:e}
% \end{subfigure}  
% \begin{subfigure}[b]{\columnwidth}
% 	\includegraphics[width=0.9\columnwidth]{Yeast05679v4.pdf}
% 	\label{fig:comp_dist:f}
% \end{subfigure}  


Different consensus

% \begin{table}[h]
%   \centering
%       \begin{adjustbox}{width=0.9\columnwidth}
%       \setlength\tabcolsep{4.0pt} 
      
%     \begin{tabular}{l c | c | c  | c  }

%     Dataset & Mean & Median & rev weighted \\
%     \hline
% \textbf{Ecoli4} & \textbf{0.188} & \textbf{0.185} & \textbf{0.185}\\
% \textbf{Glass} & 0.12 & \textbf{0.125} & \textbf{0.125}\\
% \textbf{PageBlocks} & \textbf{0.208} & 0.202 & \textbf{0.209}\\
% \textbf{Pima} & \textbf{0.037} & \textbf{0.037} & \textbf{0.037}\\
% \textbf{SatImage} & \textbf{0.792} & 0.695 & \textbf{0.793}\\
% \textbf{Shuttle} & \textbf{0.021} & \textbf{0.021} & \textbf{0.021}\\
% \textbf{SpamBase} & 0.06 & 0.059 & 0.059\\
% \textbf{Stamps} & 0.136 & \textbf{0.139} & \textbf{0.14}\\
% \textbf{Waveform} & \textbf{0.057} & 0.054 & \textbf{0.059}\\
% \textbf{WDBC} & \textbf{0.588} & \textbf{0.593} & \textbf{0.592}\\
% \textbf{Wilt} & \textbf{0.013} & \textbf{0.013} & \textbf{0.013}\\
% \textbf{WPBC} & \textbf{0.239} & \textbf{0.239} & \textbf{0.239}\\
% \textbf{Yeast05679v4} & \textbf{0.181} & \textbf{0.18} & \textbf{0.181}\\
% \textbf{Yeast2v4} & \textbf{0.447} & \textbf{0.442} & \textbf{0.443}\\
% \textbf{Average} & 0.220 & 0.213    &     0.221 
%   \end{tabular}
%   \end{adjustbox}
%   \caption{Performance under different consensus functions \label{tab:consensus}}
%   \label{consensus}
%   \vspace{-2em}
% \end{table}

Consensus comparison 


% \begin{table*}[t]
% \begin{adjustbox}{width=2\columnwidth}
% \centering
% \begin{tabular}{rrrrr}
%   \hline
%  Data set  & rev-weighted(All comps) & min-err(single comp) & upto-min-err (partial)\\
%   \hline
% \textbf{Ecoli4} & 0.173 & \textbf{0.233} & \textbf{0.207}\\
% \textbf{Glass} & \textbf{0.123} & \textbf{0.123} & \textbf{0.123}\\
% \textbf{Lympho} & \textbf{0.944} & 0.875 & \textbf{0.92}\\
% \textbf{PageBlocks} & \textbf{0.336} & \textbf{0.343} & \textbf{0.348}\\
% \textbf{Pima} & \textbf{0.035} & 0.031 & \textbf{0.034}\\
% \textbf{SatImage} & \textbf{0.618} & 0.438 & 0.534\\
% \textbf{Shuttle} & \textbf{0.022} & \textbf{0.031} & \textbf{0.031}\\
% \textbf{SpamBase} & \textbf{0.059} & \textbf{0.058} & \textbf{0.058}\\
% \textbf{Stamps} & \textbf{0.129} & \textbf{0.126} & \textbf{0.128}\\
% \textbf{WDBC} & \textbf{0.566} & \textbf{0.54} & \textbf{0.557}\\
% \textbf{Wilt} & \textbf{0.013} & 0.013 & \textbf{0.013}\\
% \textbf{WPBC} & 0.239 & \textbf{0.244} & \textbf{0.24}\\
% \textbf{Yeast05679v4} & \textbf{0.172} & 0.155 & \textbf{0.162}\\
% \textbf{Yeast2v4} & \textbf{0.359} & \textbf{0.322} & \textbf{0.33}\\
%   \hline
% \end{tabular}
% \end{adjustbox}
% \caption{  Comparison of average AUCPRs under different consensus scenarios - Fixed depth of 3 - Including consensus of iterations (rev-weighted) upto the iteration with minimum error on the sample.  Numbers are average of 30 runs and there are 20 components }
% \label{diff-consens}
% \end{table*}






% \begin{table*}[t]
% \begin{adjustbox}{width=2\columnwidth}
% \centering
% \begin{tabular}{rrrrr}
%   \hline
%  Data set  & rev-weighted(All comps) & min-err(single comp) & upto-min-err (partial)\\
%   \hline
% \textbf{Ecoli4} & 0.16 & 0.251 & 0.191\\
% \textbf{Glass} & \textbf{0.123} & \textbf{0.122} & \textbf{0.123}\\
% \textbf{Lympho} & \textbf{0.967} & 0.882 & \textbf{0.946}\\
% \textbf{PageBlocks} & 0.314 & \textbf{0.347} & \textbf{0.349}\\
% \textbf{Pima} & \textbf{0.035} & 0.03 & \textbf{0.034}\\
% \textbf{SatImage} & \textbf{0.68} & 0.451 & \textbf{0.622}\\
% \textbf{Shuttle} & 0.021 & \textbf{0.039} & \textbf{0.036}\\
% \textbf{SpamBase} & \textbf{0.059} & \textbf{0.058} & \textbf{0.059}\\
% \textbf{Stamps} & \textbf{0.127} & \textbf{0.12} & \textbf{0.126}\\
% \textbf{WDBC} & \textbf{0.567} & 0.533 & \textbf{0.571}\\
% \textbf{Wilt} & \textbf{0.013} & 0.013 & \textbf{0.013}\\
% \textbf{WPBC} & 0.239 & 0.244 & 0.239\\
% \textbf{Yeast05679v4} & \textbf{0.181} & 0.154 & \textbf{0.173}\\
% \textbf{Yeast2v4} & \textbf{0.366} & 0.319 & \textbf{0.341}\\
%   \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Comparison of average AUCPRs under different consensus scenarios - Fixed depth of 3 - Including consensus of iterations (rev-weighted) upto the iteration with minimum error on the sample.  Numbers are average of 30 runs and there are 20 components }
% \label{diff-consens}
% \end{table*}



% \begin{table*}[t]
% \begin{adjustbox}{width=2\columnwidth}
% \centering
% \begin{tabular}{rrrrr}
%   \hline
%  Data set  & rev-weighted(All comps) & min-err(single comp) & upto-min-err (partial)\\ 
%   \hline
% \textbf{Ecoli4} & \textbf{0.122} & \textbf{0.123} & \textbf{0.122}\\
% \textbf{Glass} & \textbf{0.125} & \textbf{0.126} & \textbf{0.125}\\
% \textbf{Lympho} & \textbf{0.935} & 0.828 & \textbf{0.902}\\
% \textbf{PageBlocks} & \textbf{0.206} & \textbf{0.211} & \textbf{0.214}\\
% \textbf{Pima} & \textbf{0.036} & \textbf{0.036} & \textbf{0.036}\\
% \textbf{SatImage} & \textbf{0.779} & \textbf{0.734} & \textbf{0.759}\\
% \textbf{Shuttle} & \textbf{0.021} & \textbf{0.021} & \textbf{0.021}\\
% \textbf{SpamBase} & \textbf{0.059} & \textbf{0.059} & \textbf{0.059}\\
% \textbf{Stamps} & \textbf{0.138} & \textbf{0.137} & \textbf{0.138}\\
% \textbf{WDBC} & \textbf{0.586} & 0.534 & \textbf{0.576}\\
% \textbf{Wilt} & \textbf{0.013} & \textbf{0.013} & 0.013\\
% \textbf{WPBC} & \textbf{0.237} & 0.227 & \textbf{0.235}\\
% \textbf{Yeast05679v4} & \textbf{0.163} & \textbf{0.165} & \textbf{0.154}\\
% \textbf{Yeast2v4} & \textbf{0.371} & \textbf{0.37} & \textbf{0.36}\\
%   \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Comparison of average AUCPRs under different consensus scenarios - Fixed depth of 9 - Including consensus of iterations (rev-weighted) upto the iteration with minimum error on the sample. Numbers are average of 30 runs and there are 20 components}
% \label{diff-consens}
% \end{table*}

% \begin{table*}[t]
% \begin{adjustbox}{width=2\columnwidth}
% \centering
% \begin{tabular}{rrrrr}
%   \hline
%  Data set  & rev-weighted(All comps) & min-err(single comp) & upto-min-err (partial)\\ 
%   \hline
% \textbf{Ecoli4} & \textbf{0.124} & \textbf{0.128} & \textbf{0.128}\\
% \textbf{Glass} & 0.125 & \textbf{0.126} & 0.124\\
% \textbf{Lympho} & \textbf{0.926} & \textbf{0.859} & \textbf{0.922}\\
% \textbf{PageBlocks} & \textbf{0.211} & \textbf{0.214} & \textbf{0.217}\\
% \textbf{Pima} & \textbf{0.036} & \textbf{0.036} & \textbf{0.036}\\
% \textbf{SatImage} & \textbf{0.761} & \textbf{0.736} & \textbf{0.784}\\
% \textbf{Shuttle} & \textbf{0.021} & \textbf{0.021} & \textbf{0.021}\\
% \textbf{SpamBase} & \textbf{0.059} & \textbf{0.059} & \textbf{0.059}\\
% \textbf{Stamps} & \textbf{0.138} & \textbf{0.138} & \textbf{0.139}\\
% \textbf{WDBC} & \textbf{0.589} & \textbf{0.574} & \textbf{0.584}\\
% \textbf{Wilt} & \textbf{0.013} & \textbf{0.013} & \textbf{0.013}\\
% \textbf{WPBC} & \textbf{0.236} & 0.228 & \textbf{0.231}\\
% \textbf{Yeast05679v4} & \textbf{0.155} & \textbf{0.156} & 0.145\\
% \textbf{Yeast2v4} & \textbf{0.363} & \textbf{0.371} & 0.352\\   \hline
% \end{tabular}
% \end{adjustbox}
% \caption{ Comparison of average AUCPRs under different consensus scenarios - Fixed depth of 9 - Including consensus of iterations (rev-weighted) upto the iteration with minimum error on the sample. Numbers are average of 30 runs and there are 20 components}
% \label{diff-consens}
% \end{table*}




% \begin{table}[h]
% \begin{adjustbox}{width=\columnwidth}
% \centering
% \begin{tabular}{r|r|r}
%   \hline
%  Dataset & full first layer ensemble & randomly connected first layer \\ 
%   \hline
% \textbf{Ecoli4} & \textbf{0.121} & \textbf{0.122}\\
% \textbf{Glass} & \textbf{0.125} & \textbf{0.125}\\
% \textbf{Lympho} & \textbf{0.902} & \textbf{0.894}\\
% \textbf{PageBlocks} & \textbf{0.211} & \textbf{0.209}\\
% \textbf{Pima} & \textbf{0.036} & \textbf{0.036}\\
% \textbf{SatImage} & \textbf{0.405} & \textbf{0.402}\\
% \textbf{Shuttle} & \textbf{0.02} & \textbf{0.02}\\
% \textbf{SpamBase} & \textbf{0.059} & \textbf{0.059}\\
% \textbf{Stamps} & \textbf{0.139} & \textbf{0.139}\\
% \textbf{WDBC} & \textbf{0.592} & \textbf{0.593}\\
% \textbf{Wilt} & \textbf{0.013} & \textbf{0.013}\\
% \textbf{WPBC} & \textbf{0.237} & \textbf{0.237}\\
% \textbf{Yeast05679v4} & \textbf{0.162} & \textbf{0.162}\\
% \textbf{Yeast2v4} & \textbf{0.372} & \textbf{0.372}\\
  
%   \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Studying the effect of the first iteration of the ensemble}
% \label{first_layer_res}
% \end{table}


% \begin{table}[h]
% \begin{adjustbox}{width=\columnwidth}
% \centering
% \begin{tabular}{r|r|r| r| r|r}
%   \hline
%  Dataset &  Soul All(avg)   & RandNet  & Random Opt & Full Opt & PCA based OD \\ 
%   \hline
% \textbf{Ecoli4} & 0.123 & 0.093 & 0.121 & 0.16 & \textbf{0.220} \\
% \textbf{Glass} & \textbf{0.13} & 0.092 & 0.125 & 0.123 & 0.104 \\
% \textbf{Lympho} & 0.352 & 0.839 & \textbf{0.979} & \textbf{0.967} & 0.930 \\
% \textbf{PageBlocks} & \textbf{0.425} & 0.212 & 0.23 & 0.314 & 0.314 \\
% \textbf{Pima} & 0.027 & 0.031 & \textbf{0.036} & \textbf{0.035} & 0.032 \\
% \textbf{SatImage} & 0.486 & 0.525 & \textbf{0.713} & \textbf{0.68} & 0.537 \\
% \textbf{Shuttle} & 0.174 & 0.021 & 0.021 & 0.021 & \textbf{0.186} \\
% \textbf{SpamBase} & 0.096 & 0.058 & 0.059 & 0.059 &\textbf{ 0.176} \\
% \textbf{Stamps} & 0.09 & 0.128 & \textbf{0.138} & \textbf{0.138} & 0.130 \\
% \textbf{WDBC} & \textbf{0.812} & 0.592 & 0.616 & 0.567 & 0.603 \\
% \textbf{Wilt} & \textbf{0.077} & 0.012 & 0.013 & 0.013 & 0.011 \\
% \textbf{WPBC} & 0.224 & 0.221 & \textbf{0.238} & \textbf{0.239} & 0.227 \\
% \textbf{Yeast05679v4} & 0.135 & 0.111 & 0.169 & \textbf{0.181} & 0.144 \\
% \textbf{Yeast2v4} & 0.184 & 0.261 & \textbf{0.372} & \textbf{0.371} & $0.322$ \\
%   \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Comparison with the PCA outlier detection method}
% \label{first_layer_res}
% \end{table}

s



% \begin{table*}[t]
% \begin{adjustbox}{width=2\columnwidth}
% \centering
% \begin{tabular}{rrrrr}
%   \hline
%  Data set  & Sample rev-weighted & Exclude weighted & Max-err-excluded & Min-err-sample\\ 
%   \hline
  
% \textbf{Ecoli4}  & \textbf{0.124} & \textbf{0.123} & \textbf{0.119} & \textbf{0.128}\\
% \textbf{Glass}  & 0.125 & 0.125 & \textbf{0.126} & \textbf{0.126}\\
% \textbf{Lympho}  & \textbf{0.926} & \textbf{0.91} & 0.817 & \textbf{0.859}\\
% \textbf{PageBlocks} & \textbf{0.211} & \textbf{0.208} & 0.203 & \textbf{0.214}\\
% \textbf{Pima}  & \textbf{0.036} & \textbf{0.036} & \textbf{0.037} & \textbf{0.036}\\
% \textbf{SatImage}  & \textbf{0.761} & 0.59 & 0.447 & \textbf{0.736}\\
% \textbf{Shuttle}  & \textbf{0.021} & \textbf{0.021} & \textbf{0.02} & \textbf{0.021}\\
% \textbf{SpamBase} & \textbf{0.059} & \textbf{0.059} & \textbf{0.059} & \textbf{0.059}\\
% \textbf{Stamps}  & \textbf{0.138} & \textbf{0.138} & \textbf{0.137} & \textbf{0.138}\\
% \textbf{WDBC}  & \textbf{0.589} &\textbf{0.59} & \textbf{0.596} & \textbf{0.574}\\
% \textbf{Wilt}  & \textbf{0.013} & \textbf{0.013} & 0.012 & \textbf{0.013}\\
% \textbf{WPBC}  &  \textbf{0.236} & \textbf{0.236} & \textbf{0.238} & 0.228\\
% \textbf{Yeast05679v4}  & \textbf{0.155} & \textbf{0.155} & \textbf{0.151} & \textbf{0.156}\\
% \textbf{Yeast2v4}  & \textbf{0.363} & 0.362 & \textbf{0.375} & \textbf{0.371}\\
  
%   \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Comparison of average AUCPRs under different consensus scenarios- fixed depth 9}
% \label{diff-consens}
% \end{table*}



% \begin{table}[h]
% \begin{adjustbox}{width=\columnwidth}
% \centering
% \begin{tabular}{rrr}
%   \hline
%   Dataset & top 3 eigen vectors &  bottom 3 eigen vectors  \\
%   \hline
% Ecoli4 & 0.21 & 0.204 \\
% Glass & 0.095 & 0.105 \\
% Lympho & 0.911 & 0.931 \\
% PageBlocks & 0.308 & 0.315 \\
% Pima & 0.027 & 0.035 \\
% SatImage & 0.559 & 0.537 \\
% Shuttle & 0.213 & 0.186 \\
% SpamBase & 0.173 & 0.176 \\
% Stamps & 0.134 & 0.131 \\
% WDBC & 0.611 & 0.604 \\
% WPBC & 0.227 & 0.227 \\
% Wilt & 0.012 & 0.012 \\
% Yeast05679v4 & 0.114 & 0.162 \\
% Yeast2v4 & 0.327 & 0.322 \\
% \hline
% \end{tabular}
% \end{adjustbox}
% \caption{AUCPR values from PCA based outlier detection method. Comparison of the effect of the top and bottom eigen vectors}
% \label{mnist-results}
% \end{table}



%\section{Results}
%\input{perf-tables.tex}


% \begin{table}[h]
% \begin{adjustbox}{width=0.8\columnwidth}
% \centering
% \begin{tabular}{rrrr}
%   \hline
%  Dataset &  Soul All(avg)   & RandNet &  Full opt
% \\ 
%   \hline
% \textbf{Ecoli4} & 0.123 & 0.093 & \textbf{0.16}\\
% \textbf{Glass} & \textbf{0.13} & 0.092 & 0.123\\
% \textbf{PageBlocks} & \textbf{0.425} & 0.212 & 0.314\\
% \textbf{Pima} & 0.027 & 0.031 & \textbf{0.035}\\
% \textbf{SatImage} & 0.486 & 0.525 & \textbf{0.68}\\
% \textbf{Shuttle} & \textbf{0.174} & 0.021 & 0.021\\
% \textbf{SpamBase} & \textbf{0.096} & 0.058 & 0.059\\
% \textbf{Stamps} & 0.09 & 0.128 & \textbf{0.138}\\
% \textbf{WDBC} & \textbf{0.812} & 0.592 & 0.567\\
% \textbf{Wilt} & \textbf{0.077} & 0.012 & 0.013\\
% \textbf{WPBC} & 0.224 & 0.221 & \textbf{0.239}\\
% \textbf{Yeast05679v4} & 0.135 & 0.111 & \textbf{0.181}\\
% \textbf{Yeast2v4} & 0.184 & 0.261 & \textbf{0.371}\\
% \hline
% \end{tabular}
% \end{adjustbox}
% \caption{RandNet vs. Selected fullyconnected autoencoders with depth of 3 and 9}
% \label{rand_vs_full}
% \end{table}



% \begin{table}[h]
% \begin{adjustbox}{width=\columnwidth}
% \centering
% \begin{tabular}{rrrrrrr}
%   \hline
% Datasets & FullSampling3 & FullSampling9 & OCSVM & IF & LOF\\
% \hline
% \textbf{0} & \textbf{0.754} & \textbf{0.763} & 0.496 & 0.469 & 0.189\\
% \textbf{1} & \textbf{0.96} & \textbf{0.956} & 0.9 & 0.922 & 0.143\\
% \textbf{2} & 0.448 & \textbf{0.511} & 0.275 & 0.238 & 0.173\\
% \textbf{3} & 0.48 & \textbf{0.554} & 0.374 & 0.338 & 0.199\\
% \textbf{4} & 0.635 & \textbf{0.693} & 0.468 & 0.419 & 0.242\\
% \textbf{5} & 0.434 & \textbf{0.589} & 0.233 & 0.233 & 0.281\\
% \textbf{6} & 0.683 & \textbf{0.721} & 0.428 & 0.348 & 0.234\\
% \textbf{7} & \textbf{0.719} & \textbf{0.733} & 0.528 & 0.541 & 0.183\\
% \textbf{8} & 0.332 & \textbf{0.418} & 0.275 & 0.21 & 0.177\\
% \textbf{9} & 0.6 & \textbf{0.65} & 0.415 & 0.376 & 0.282\\   \hline
% \end{tabular}
% \end{adjustbox}
% \caption{MNIST dataset results under two different sizes of Autoencoders. 20 components in each ensemble. Rev-weighted is used as consensus. Numbers are averages of 20 runs}
% \label{mnist-results}
% \end{table}



% \begin{table}[h]
% \begin{adjustbox}{width=\columnwidth}
% \centering
% \begin{tabular}{rrrrrrrr}
%   \hline
%   Data sets & BAE-3 & BAE-9 & RandNet & OCSVM & IF & LOF & SimpleAE \\
%   \hline
% \textbf{0} & \textbf{0.754} & \textbf{0.763} & 0.180 & 0.496 & 0.469 & 0.189 & 0.189\\
% \textbf{1} & \textbf{0.96} & \textbf{0.956} & 0.77 & 0.9 & 0.922 & 0.143 & 0.143\\
% \textbf{2} & 0.448 & \textbf{0.511} & 0.109 & 0.275 & 0.238 & 0.173 & 0.173\\
% \textbf{3} & 0.48 & \textbf{0.554} & 0.082 &0.374 & 0.338 & 0.199 & 0.199\\
% \textbf{4} & 0.635 & \textbf{0.693} &0.104 &0.468 & 0.419 & 0.242 & 0.242\\
% \textbf{5} & 0.434 & \textbf{0.589} & 0.070 & 0.233 & 0.233 & 0.281 & 0.281\\
% \textbf{6} & 0.683 & \textbf{0.721} & 0.184 & 0.428 & 0.348 & 0.234 & 0.234\\
% \textbf{7} & \textbf{0.719} & \textbf{0.733} & 0.348 & 0.528 & 0.541 & 0.183 & 0.183\\
% \textbf{8} & 0.332 & \textbf{0.418} & 0.089 & 0.275 & 0.21 & 0.177 & 0.177\\
% \textbf{9} & 0.6 & \textbf{0.65} & 0.295 & 0.415 & 0.376 & 0.282 & 0.282\\
  
  
%   \hline
% \end{tabular}
% \end{adjustbox}
% \caption{MNIST data set results under two different sizes of Autoencoders. 20 components in each ensemble. Rev-weighted is used as consensus. Numbers are averages of 20 runs}
% \label{mnist-results}
% \end{table}


% \begin{table}[h]
% \begin{adjustbox}{width=0.8\columnwidth}
% \centering
% \begin{tabular}{rrr}
%   \hline
%  Dataset & RandNet & Fullyconnected opt \\ 
%   \hline
%   \textbf{Ecoli4} & 0.093 & \textbf{0.16}\\
% \textbf{Glass} & 0.092 & \textbf{0.123}\\
% \textbf{Lympho} & 0.839 & \textbf{0.967}\\
% \textbf{PageBlocks} & 0.212 & \textbf{0.314}\\
% \textbf{Pima} & 0.031 & \textbf{0.035}\\
% \textbf{SatImage} & 0.525 & \textbf{0.68}\\
% \textbf{Shuttle} & \textbf{0.021} & 0.021\\
% \textbf{SpamBase} & 0.058 & \textbf{0.059}\\
% \textbf{Stamps} & 0.128 & \textbf{0.138}\\
% \textbf{WDBC} & \textbf{0.592} & 0.567\\
% \textbf{Wilt} & 0.012 & \textbf{0.013}\\
% \textbf{WPBC} & 0.221 & \textbf{0.239}\\
% \textbf{Yeast05679v4} & 0.111 & \textbf{0.181}\\
% \textbf{Yeast2v4} & 0.261 & \textbf{0.371}\\
  
%   \hline
% \end{tabular}
% \end{adjustbox}
% \caption{RandNet vs. Selected fullyconnected autoencoders with depth of 3 and 9}
% \label{rand_vs_full}
% \end{table}





% \begin{table}[h]
%   \centering
%   %   \begin{adjustbox}{width=0.9\columnwidth}
%       \setlength\tabcolsep{4.0pt} 
%     \begin{tabular}{l c | c | c  }

%     Data set & 20 comps & 100 comps & 200 comps \\
%     \hline
% \textbf{Ecoli4} & \textbf{0.122} & \textbf{0.12} & 0.12\\
% \textbf{Glass} & \textbf{0.125} & \textbf{0.125} & \textbf{0.125}\\
% \textbf{PageBlocks} & \textbf{0.209} & 0.203 & 0.203\\
% \textbf{Pima} & \textbf{0.036} & \textbf{0.036} & \textbf{0.036}\\
% \textbf{SatImage} & \textbf{0.402} & 0.384 & 0.38\\
% \textbf{Shuttle} & \textbf{0.02} & \textbf{0.02} & \textbf{0.02}\\
% \textbf{SpamBase} & \textbf{0.059} & 0.059 & 0.059\\
% \textbf{Stamps} & \textbf{0.139} & \textbf{0.138} & \textbf{0.138}\\
% \textbf{Waveform} & \textbf{0.055} & \textbf{0.055} & \textbf{0.055}\\
% \textbf{WDBC} & \textbf{0.593} & \textbf{0.593} & \textbf{0.593}\\
% \textbf{Wilt} & \textbf{0.013} & 0.013 & 0.013\\
% \textbf{WPBC} & 0.237 & \textbf{0.238} & \textbf{0.238}\\
% \textbf{Yeast05679v4} & 0.162 & \textbf{0.166} & \textbf{0.166}\\
% \textbf{Yeast2v4} & 0.372 & \textbf{0.377} & \textbf{0.377}\\
% \textbf{Average} & 0.181 &  0.180 & 0.180 
%   \end{tabular}
%   %\end{adjustbox}
%   \caption{{\color{red} Change to box plots for the same 4 datasets}Performance of the sampling method under different number of ensemble components \label{tab:consensus}}
%   \vspace{-2em}
%   \label{ens-size}
% \end{table}





% \begin{table*}[h]
% %\begin{adjustbox}{width=\textwidth}
% \centering
% \begin{tabular}{c|c c c c c c}
%   \hline
%   Data set & LOF & AE & OCSVM & Hawkins & RandNet & BAE\\
%   \hline
% \textbf{MNIST0} & 0.189 & 0.661 & 0.496 & 0.463 & \textbf{0.713} & \textbf{0.718}\\
% \textbf{MNIST1} & 0.143 & 0.921 & 0.9 & 0.937 & 0.947 & \textbf{0.966}\\
% \textbf{MNIST2} & 0.173 & 0.427 & 0.275 & 0.37 & 0.436 & \textbf{0.515}\\
% \textbf{MNIST3} & 0.199 & 0.456 & 0.374 & 0.451 & 0.474 & \textbf{0.548}\\
% \textbf{MNIST4} & 0.242 & 0.577 & 0.468 & 0.516 & \textbf{0.676} & \textbf{0.667}\\
% \textbf{MNIST5} & 0.281 & 0.497 & 0.233 & 0.488 & 0.495 & \textbf{0.594}\\
% \textbf{MNIST6} & 0.234 & 0.675 & 0.428 & 0.533 & 0.706 & \textbf{0.743}\\
% \textbf{MNIST7} & 0.183 & 0.669 & 0.528 & 0.597 & 0.698 & \textbf{0.72}\\
% \textbf{MNIST8} & 0.177 & 0.328 & 0.275 & \textbf{0.403} & 0.394 & \textbf{0.412}\\
% \textbf{MNIST9} & 0.282 & 0.608 & 0.415 & 0.506 & 0.648 & \textbf{0.675}\\
%   \hline
% \end{tabular}
% %\end{adjustbox}
% \caption{Comparison of \algo with other baselines on MNIST dataset. Average area under PR curve for 30 runs of each method is reported.}
% \label{mnist-results}
% \end{table*}
